Meta-learning for mixed linear regression

In modern supervised learning, there are a large number of tasks, but many of them are associated with only a small amount of labeled data. These include data from medical image processing and robotic interaction. Even though each individual task cannot be meaningfully trained in isolation, one seeks to meta-learn across the tasks from past experiences by exploiting some similarities. We study a fundamental question of interest: When can abundant tasks with small data compensate for lack of tasks with big data? We focus on a canonical scenario where each task is drawn from a mixture of $k$ linear regressions, and identify sufficient conditions for such a graceful exchange to hold; The total number of examples necessary with only small data tasks scales similarly as when big data tasks are available. To this end, we introduce a novel spectral approach and show that we can efficiently utilize small data tasks with the help of $\tilde\Omega(k^{3/2})$ medium data tasks each with $\tilde\Omega(k^{1/2})$ examples.

==> Meta-Learning Linear Regression_ k-Mixture/abstract.tex <==
% weihao
%In many setting lots of data from heterogeneous tasks, each task has a small amount of data. Learning is impossible for each task separately. Meta-learning address this setting.
%Despite empirical success, few theoretically results are known about to what extent can the large number of prior data sources help with inference for the new task.

 %Meta-learning addresses an important challenge i

In modern supervised learning, there are a large number of tasks, but many of them are associated with only a small amount of labelled data. These include data from medical image processing and robotic interaction. 
Even though each individual task cannot be meaningfully trained in isolation, 
 one seeks to meta-learn across the tasks from past experiences by exploiting some similarities. 
We study a  fundamental question of interest: 
When can abundant tasks with small data compensate for lack of tasks with big data? 
 We focus on a canonical scenario where each task is drawn from a mixture of $k$ linear regressions, 
 and identify sufficient conditions for such a graceful exchange to hold; The total number of examples necessary with only small data tasks scales similarly as when big data tasks are available.
 To this end, we introduce a novel spectral approach and 
 show that we 
 can efficiently utilize small data tasks with the help of $\tilde\Omega(k^{3/2})$ medium data tasks each with $\tilde\Omega(k^{1/2})$ examples.

% This is achieved by introducing a novel spectral algorithm and analyzing the sample complexity involved in each step.  
%We study the classical mixed liner regression model in the meta learning setting...proposed efficient and practical algorithm for parameter estimation.... comparing to previous work on mixed linear regression, our algorithm achieves near optimal complexity by using a small number of tasks that has relatively large amount of data. use heavy tasks and light tasks, fit for many practical scenario... 
%we characterized the benefit one can achieve through meta learning, and the interplay between the number of priors tasks, and the informatio per task...


==> Meta-Learning Linear Regression_ k-Mixture/algo_details.tex <==
\section{Details of the algorithm and the analyses}
\label{sec:algorithm_detail}

We explain and analyze  each step in  Algorithm \ref{alg:estimate}. 
These analyses  imply our main result in meta-learning, which is explicitly written in Appendix~\ref{sec:proof_est}.

\subsection{Subspace estimation} 

In the following, we use  $k$\_SVD$(\cdot, k)$ routine that outputs the top $k$-singular vectors.
As ${\mathbb E}[{\hat\M}] = 
\M :=\sum_{j=1}^k p_j \w_j\w_j^\top$, 
this outputs an estimate of the subspace spanned by the true parameters. 
We show that as long as $t_{L1}\geq 2$, the accuracy only depends on the total 
number of examples, and it is sufficient to have 
$n_{L1}t_{L1}=\tilde{\Omega}(d)$.  

\begin{algorithm}[h]
   \caption{Subspace estimation}
   \label{alg:subspace_estimation}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $\Dcal_{L1} = \curly{(\x_{i,j},y_{i,j})}_{i\in[n_{L1}],j\in[t_{L1}]}$, $k\in\Natural$
%   \REPEAT
%   \STATE Initialize $noChange = true$.
   \STATE {\bf compute} for all $i\in[n_{L1}]$ 
   %\FOR{$i=1$ {\bfseries to} $n_{L1}$}
   \STATE \hspace{-.5cm} $\hat{\beta}^{(1)}_i \gets \frac{2}{t_{L1}}\sum\limits_{j=1}^{t_{L1}/2}y_{i,j}\x_{i,j}$,\ $\hat{\beta}^{(2)}_i \gets \frac{2}{t_{L1}}\sum\limits_{j=t_{L1}/2+1}^{t_{L1}}y_{i,j}\x_{i,j}$
%   \IF{$x_i > x_{i+1}$}
%   \STATE Swap $x_i$ and $x_{i+1}$
%   \STATE $noChange = false$
%   \ENDIF
   %\ENDFOR
   \STATE $\hat\M \gets \round{2n_{L1}}^{-1}\sum_{i=1}^{n_{L1}} \round{\hat\beta_i^{(1)}\hat\beta_i^{(2)\top} + \hat\beta_i^{(2)}\hat\beta_i^{(1)\top}}$
   \STATE $\U \gets $ $k$\_SVD$\round{\hat\M,k}$
%   \UNTIL{$noChange$ is $true$}
    \OUTPUT $\U$
\end{algorithmic}
\end{algorithm}


The dependency on the accuracy $\eps$ changes based on the ground truths meta-parameters. 
In an ideal case when $\W$ is an orthonormal matrix (with condition number one), the sample complexity is $\tilde{\Ocal}\round{d/(p_{\rm min}^2 \varepsilon^2) }$. 
For the worst case $\W$, 
it is $\tilde{\Ocal}\round{d/\round{p_{\rm min}^2\varepsilon^6}}$. 
% The standard deviation  $\rho$ of the labels captures the scaling of the problem parameters, and we normalize the error by $\rho$. 
%\Weihao{There is something wrong in our proof. We showed concentration the $\beta$ matrix instead of $w$ matrix, and $\lambda_{min}$ should be for the $\beta$ matrix as well. How are the two $\lambda_{min}$ related?}\Raghav{Lemma~\ref{lem:bound_X_Xbar}?}

\begin{lemma}[Learning the subspace]
\label{lem:projection}
Suppose Assumption~\ref{asmp} holds, and let $\U\in \Rd{d\times k}$ be the matrix with top $k$ eigen vectors of matrix $\hat\M\in{\mathbb R}^{d\times d}$. For any failure probability   $\delta \in (0,1)$ and accuracy $\eps \in (0,1)$, if the sample size is large enough such that 
\begin{align*}
%n_{L1} &= \Omega \round{  d t_{L1}^{-1}\cdot \min \curly{ \eps^{-6} p_{\min}^{-2} , \eps^{-2} \lambda_{\min}^{-2} \rho^4 } \cdot \log^3(nd/\delta)},
n_{L1} &= \Omega \round{  d t_{L1}^{-1}\cdot \min \curly{ \eps^{-6} p_{\min}^{-2} , \eps^{-2} \lambda_{\min}^{-2}  } \cdot \log^3(nd/\delta)},
\end{align*} 
and $2 \leq t_{L1} <d$, we have 
\begin{align}\label{eq:projection}
%\frac{1}{\rho}
\enorm{(\U\U^\top-\I) \w_i} \;\; \le \;\; \eps\quad,
\end{align}
for all $i\in[k]$ 
with probability at least $1-\delta$, where $\lambda_{\rm min}$ is the smallest non-zero eigen value of $\M:=\sum_{j=1}^k p_j \w_j\w_j^\top$. 
%and $\rho^2=\max_{i\in[k]} s_i^2 + \|\w_i\|_2^2$ is the maximum variance of the label. 
\end{lemma}

{\textbf{Time complexity:}} 
%Note that $\hat\M$ can be computed as
% First we analyze the time complexity for constructing the estimator $\hat{\M}$. To speed up the computation, we can use matrix multiplication and compute $\hat{\M}$ with 
%\begin{align*}
%\B^{(1)}&\gets \begin{bmatrix}\hat{\beta}^{(1)}_1&\ldots&\hat{\beta}^{(1)}_{n_{L1}}\end{bmatrix},\; \B^{(2)} \gets \begin{bmatrix}\hat{\beta}^{(2)}_1&\ldots&\hat{\beta}^{(2)}_{n_{L1}}\end{bmatrix}\\
%\hat\M &\gets \round{2n_{L1}}^{-1}\B^{(1)}\B^{(2)\top}+\B^{(2)}\B^{(1)\top}.
%\end{align*}
 $\BigO{\round{n_{L1}^{\omega-1}+n_{L1}t_{L1}}d}$ 
  for 
 computing $\hat\M$, and $\BigO{kd^2}$  for $k$\_SVD 
\cite{AL16}.



\subsection{Clustering}

Once we have the subspace, we can efficiently cluster any 
 task associated with  $t_H=\tilde\Omega(\sqrt{k})$ samples. 
In the following, the matrix $\Hmat \in{\mathbb R}^{n_H\times n_H}$ estimates 
the distance between the parameters in the projected $k$-dimensional space. 
If there is no error in $\U$, then ${\mathbb E}[\Hmat_{i,j}]\geq \Omega\round{\Delta^2}$ if $i$ and $j$ are from different components, and zero otherwise. 
Any clustering algorithm can be applied treating $\Hmat$ as a distance matrix.
% Our analysis holds for a specific choice of  \Sewoong{explain our clustering, is it single linkage?? or just thresholding?? }

%any non-degenerate clustering algorithm that returns the correct clusters when applied to a graph with $k$ disjoint cliques. 

% which can be any algorithm which takes in a pair-wise distance matrix and outputs the cluster.

\begin{algorithm}[h]
   \caption{Clustering and estimation}
   \label{alg:clustering}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $\Dcal_H = \curly{(\x_{i,j},y_{i,j})}_{i\in[n_H],j\in[t_H]}$, $2L\leq t_H$, $k\in\Natural$, $L\in\Natural$, $\U\in\Rd{d\times k}$
   \STATE {\bf compute} for all $\ell\in[L]$ and $i\in[n_H]$
    \STATE \hspace{0.3cm}  $\beta^{(\ell)}_i \gets \round{\nicefrac{2L}{t_H}}\sum_{j=(\ell-1)\cdot\round{\nicefrac{t_H}{2L}}+1}^{\ell\cdot\round{\nicefrac{t_H}{2L}}}y_{i,j}\x_{i,j}$
        \STATE \hspace{0.3cm}  $\beta^{(\ell+L)}_i \gets \round{\nicefrac{2L}{t_H}}\sum_{j=\ell \cdot\round{\nicefrac{t_H}{2L}}+1}^{2\ell \cdot\round{\nicefrac{t_H}{2L}}}y_{i,j}\x_{i,j}$
   \STATE {\bf compute} for all $\ell\in[L]$ and $(i,j)\in[n_H]\times [n_H]$
%   \FOR{$l=1$ {\bfseries to} $L$}
 %       \FOR{$(i,j)\in\squarebrack{n_2}\times\squarebrack{n_2}$}
            \STATE \hspace{0.3cm} $\Hmat_{i,j}^{(\ell)} \gets \round{\hat\beta_i^{(\ell)} - \hat\beta_j^{(\ell)}}^\top\U \U^\top\round{\hat\beta_i^{(\ell+L)} - \hat\beta_j^{(\ell+L)}}$
            %\Sewoong{$\ell'$ is not defined, acn you change all $l$ to $\ell$?}
%        \ENDFOR
%   \ENDFOR
%   \FOR{$(i,j)\in\squarebrack{n_2}\times\squarebrack{n_2}$}
    \STATE {\bf compute} for all $(i,j)\in[n_H] \times [n_H]$
        \STATE \hspace{0.3cm} $\Hmat_{i,j} \gets $ median$\round{ \{\Hmat_{i,j}^{(\ell)}\}_{\ell\in[L]}}$
%    \ENDFOR
   \STATE Cluster $\Dcal_H$ using $\Hmat$ and return its partition $\curly{\Ccal_\ell}_{\ell\in[k]}$
    %\FOR{$l=1$ {\bfseries to} $k$}
    \STATE {\bf compute} for all $\ell\in[L]$
         \STATE \hspace{0.3cm} $\tilde\w_\ell \gets \round{t_H \abs{\Ccal_\ell}}^{-1}
         \sum_{i\in\Ccal_\ell,j\in[t_H]}\,
         y_{i,j}\U\U^\top\x_{i,j}$
         \STATE \hspace{0.3cm} $\tilde{r}_\ell^2 \gets \round{t_H\abs{\Ccal_\ell}}^{-1}
         \sum_{i\in\Ccal_\ell,j\in[t_H]}\,
         \round{y_{i,j}-\x_{i,j}^\top\tilde\w_\ell}^2$
        \STATE \hspace{0.3cm} $\tilde{p}_\ell \gets \abs{\Ccal_\ell}/n_H$
    %\ENDFOR
    \OUTPUT $\curly{\Ccal_\ell,\; \tilde\w_\ell,\; \tilde{r}^2_\ell,\; \tilde{p}_\ell}_{\ell=1}^k$
\end{algorithmic}
\end{algorithm}



This is inspired by \cite{vempala2004spectral}, where 
clustering mixture of Gaussians is studied.
One might wonder if it is possible to apply their clustering approach to $\hat{\beta}_i$'s directly. This approach fails as it crucially relies on the fact that 
%with for $\x \sim \cal N(\mu, \I)$, it holds that 
$\enorm{\x-\mu} = \sqrt{k}\pm\tilde\Ocal(1)$ with high probability for $\x\sim \N(\zero,\I_k)$.
Under our linear regression setting, $\enorm{y\x-\beta}$ does not concentrate. 
We instead propose median of estimates, to get the desired $t_H=\tilde\Omega(\sqrt{k})$ sufficient condition. 

%\begin{figure}[ht]
%    \vskip 0.2in
%    \begin{center}
%    \subfigure[Without median of estimates]{\label{fig:hist_overlap}\includegraphics[width=.49\linewidth]{images/hist_mean.png}}
%    \subfigure[With median of estimates]{\label{fig:hist_separate}\includegraphics[width=.49\linewidth]{images/hist_median.png}}
%    \caption{Histogram of $\curly{\Hmat_{i,j}}_{i,j\in\squarebrack{n}\times\squarebrack{n}}$ illustrates that median improves the concentration of the distance estimates. \Raghav{Had to use poly-tail distributions like $\x_{i,j},\eps_{i,j}\sim p(x)\propto\inv{\abs{x}^4}$ to observe better concentration of median for $d=k=3$.}}
%    \label{fig:median}
%    \end{center}
%    \vskip -0.2in
%\end{figure}


\begin{lemma}[Clustering and initial parameter estimation]
\label{lem:distance}
Under Assumption~\ref{asmp}, and given an orthonormal matrix $\U\in{\mathbb R}^{d\times k}$ satisfying 
\eqref{eq:projection} with any  %$\eps\in\round{0,{\nicefrac{\Delta}{4\rho}}}$,
$\eps\in\round{0,{\nicefrac{\Delta}{4}}}$, Algorithm~\ref{alg:clustering} correctly clusters all tasks  with 
%$t_H = \Omega\round{\rho^2\Delta^{-2}\sqrt{k}\log({n}/{\delta})}=\BigO{k}$ 
$t_H = \Omega( \Delta^{-2}\sqrt{k}\log({n}/{\delta}))$ 
 with probability at least $1-\delta$, $\ \forall\ \delta\in\round{0,1}$. 
Further, if
% and $\tilde\eps\in\round{0,\sqrt{p_{\rm min}k/t}}$ and if 
\begin{eqnarray}
%n \;\; =\;\; \Omega\round{\frac{\Delta^2 \, \sqrt{k}}{p_{\rm min}(\rho\tilde\eps)^2\,\log\round{\nicefrac{k}{\eps\delta}}}}\;,
n_H \;\; =\;\; \Omega\round{\frac{  k\, \log(k/\delta)}{t_H\,\tilde\eps^2\,p_{\rm min}}}\;, 
\end{eqnarray}
  for any $\tilde\eps>0$, with probability at least $1-\delta$, 
  \begin{subequations}
    \begin{eqnarray}
    %\abs{\hat{p}_i-p_i}&\leq& \tilde\eps\sqrt{\frac{p_{\rm min}t}{k}}\\
    %\esqnorm{\U^\top(\hat\w_i-\w_i)} &\leq& \tilde\eps\rho\\
    \esqnorm{\U^\top(\tilde\w_i-\w_i)} &\leq& \tilde\eps \\
    \abs{\tilde{r}_i^2 - r_i^2} &\leq& \frac{\tilde\eps}{\sqrt{k}}r_i^2 \;,
  \end{eqnarray}
  \end{subequations}
where $r_i^2 \coloneqq (s_i^2 + \esqnorm{\tilde\w_i-\w_i})$ for all $ i\in\squarebrack{k}$.
%and  $\hat{\w}_i$ and $\hat{r}_i^2$ are computed according to Algorithm~\ref{alg:clustering}.
\end{lemma}
{\textbf{Time complexity:}} It takes $\BigO{n_Hdt_H+n_Hdk}$ time to compute $\{\U^\top\hat{\beta}_i^{(l)}\}_{i\in\squarebrack{n_H},l\in\squarebrack{L}}$. Then by using matrix multiplication, it takes $\BigO{n_H^2 k^{\omega-2}}$ time to compute the matrix $\Hmat$, and the single linkage clustering algorithm takes $\BigO{n_H^2}$ time~\cite{sibson1973slink}.


\subsection{Classification}

Once we have $\curly{\tilde\w_\ell}_{\ell=1}^k$ from the clustering step, we can efficiently classify any task with $t_{L2}=\tilde\Omega(\log k)$ samples, and an extra $\log n_{L2}$ samples are necessary to apply the union bound. 
This allows us to use the light samples, in order to refine the  clusters estimated with heavy samples. This separation allows us to achieve the desired sample complexity on light tasks $(t_{L2}=\Omega(\Delta^{-4}\log d),n_{L2}t_{L2}p_{\rm min}=\tilde\Omega(\epsilon^{-2}d))$, and heavy tasks $(t_H=\tilde\Omega(\Delta^{-2}\sqrt{k}),n_Ht_Hp_{\rm min}=\tilde\Omega(\Delta^{-2} k))$. %Without the separation, we would require one batch of samples with  $t_{L2}=\tilde\Omega(\Delta^{-2}\sqrt{k})$, and $n_{L2}t_{L2}p_{\rm min}=\tilde\Omega(\epsilon^{-2} d)$.

In the following, we use Least\_Squares$(\cdot)$ routine that outputs the least-squares estimate of all the examples in each cluster. Once each cluster has $\BigO{d}$ samples, we can accurately estimate the meta-parameters. 

 

\begin{algorithm}[h]
   \caption{Classification and estimation}
   \label{alg:classification}
\begin{algorithmic}
   \STATE {\bfseries Input:} data $\Dcal_{L2} =  \curly{(\x_{i,j},y_{i,j})}_{i\in[n_{L2}],j\in[t_{L2}]}$, $\curly{\Ccal_\ell,\; \tilde\w_\ell,\; \tilde{r}^2_\ell }_{\ell\in[k]}$
   \STATE {\bf compute} for all $i\in[n_{L2}]$ 
    $$h_i \gets \argmin_{\ell \in\squarebrack{k}} 
    \inv{2\tilde{r}_\ell^2}\sum_{j\in\squarebrack{t_{L2}}} \round{y_{i,j}-\x_{i,j}^\top\tilde\w_\ell}^2 + t_{L2} \log\tilde{r}_\ell$$
%   \FOR{$i=1$ {\bfseries to} $n_3$}
%        \FOR{$l=1$ {\bfseries to} $k$}
%      \STATE \hspace{0.3cm} $\hat{l}_i \gets - \inv{2\hat{r}_l^2}\sum_{j\in\squarebrack{t_3}} \round{y_{i,j}-\x_{i,j}^\top\hat\w_l}^2 - t_{L2} \log\hat{r}_l$
%        \ENDFOR
        \STATE \hspace{0.3cm}  $\Ccal_{h_i}\gets \Ccal_{h_i}\cup\curly{(\x_{i,j},y_{i,j})}_{j=1}^{t_{L2}}$
%   \ENDFOR
    %\FOR{$l=1$ {\bfseries to} $k$}
    \STATE {\bf compute} for all $\ell\in[k]$, 
        \STATE \hspace{0.3cm} $\hat\w_\ell \gets$ Least\_Squares$(\Ccal_\ell)$
        \STATE \hspace{0.3cm} $\hat{s}_\ell^2 \gets \round{t_{L2} \abs{\Ccal_\ell}-d}^{-1}
        \sum_{i \in\Ccal_\ell,j\in[t_{L2}]}
        \round{y_{i,j}-\x_{i,j}^\top\hat\w_\ell}^2 $
        \STATE \hspace{0.3cm} $\hat{p}_\ell \gets \abs{\Ccal_\ell}/n_{L2}$
    %\ENDFOR
    \OUTPUT $\curly{\Ccal_\ell,\; \hat\w_\ell,\; \hat{s}^2_\ell,\; \hat{p}_\ell}_{\ell=1}^k$
\end{algorithmic}
\end{algorithm}

\begin{lemma}[Refined parameter estimation via classification]\label{lem:refined-est}
Under Assumption~\ref{asmp} and given estimated parameters $\tilde{\w}_i$, $\tilde{r}_i$ satisfying $\enorm{\tilde{\w}_i-\w_i} \le \Delta/10$,  %$\round{1-\Delta^2/50\rho^2}\hat{r}_i^2\le s_i^2+\esqnorm{\hat{\w}'_i-\w_i}\le \round{1+\Delta^2/50\rho^2}\hat{r}_i^2$ for all $i\in [k]$ and 
$\round{1-\Delta^2/50}\tilde{r}_i^2\le s_i^2+\esqnorm{\tilde{\w}_i-\w_i}\le \round{1+\Delta^2/50}\tilde{r}_i^2$ for all $i\in [k]$ and 
$n_{L2}$ task with $t_{L2} = \Omega\round{\log (k n_{L2}/\delta)/\Delta^4}$ examples per task, with probability $1-\delta$, Algorithm~\ref{alg:classification} correctly classifies all the $n_{L2}$ tasks. Further, for any $0 <\eps \le 1$ if 
\begin{eqnarray}
%n \;\; =\;\; \Omega\round{\frac{\Delta^2 \, \sqrt{k}}{p_{\rm min}(\rho\tilde\eps)^2\,\log\round{\nicefrac{k}{\eps\delta}}}}\;,
n_{L2} \;\; =\;\; \Omega\round{\frac{  \,d \log^2(k/\delta)}{t_{L2} p_{\rm min}\eps^2 }}\;, 
\end{eqnarray}
the following holds for all $i\in[k]$, 
\begin{subequations}
\label{eq:estimation_err}
\begin{eqnarray}
\enorm{\hat{\w}_i-\w_i} &\le& \eps s_i\; , \\ 
\abs{\hat{s}_i^2-s_i^2}&\le&  \frac{\eps}{\sqrt{d}}s_i^2\; ,\quad\text{and}\\
\abs{\hat{p}_i-p_i} &\le&  \eps \sqrt{t_{L2}/d}\,p_i.
\end{eqnarray}
\end{subequations}
\end{lemma}
{\textbf{Time complexity:}} Computing $\{h_i\}_{i\in\squarebrack{n_{L2}}}$ takes $\BigO{n_{L2}t_{L2}dk}$ time, and least square estimation takes $\BigO{n_{L2}t_{L2}d^{\omega-1}}$ time.

%\subsection{Prediction}


%\begin{algorithm}[tb]
%   \caption{Prediction}
%   \label{alg:prediction}
%\begin{algorithmic}
%   \STATE {\bfseries Input:} data $\Tcal = \curly{\x_{j},y_{j}}_{j=1}^{\tau}$, $\curly{\Ccal_l,\; \hat\w_l,\; \hat{s}^2_l,\; \hat{p}_l}_{l=1}^k$
%    \FOR{$l=1$ {\bfseries to} $k$}
%        \STATE $\hat{L}_l \gets \exp\round{\frac{-1}{2\hat{s}_l^2}\sum\limits_{j\in\squarebrack{\tau}}\round{y_{j}-\x_{j}^\top\hat\w_l}^2 - \tau\log\hat{s}_l + \log \hat{p}_l}$
%    \ENDFOR
%    \STATE $\hat{i} \gets \argmax\limits_{l\in\squarebrack{k}}\hat{L}_l$, \; $\beta_{\rm Bayes} \gets \frac{\sum_{l\in\squarebrack{k}} \hat{L}_l\hat\w_l}{\sum_{l\in\squarebrack{k}} \hat{L}_l}$, \; $\beta_{\rm MAP} \gets \hat\w_{\hat{i}}$
%    \FOR{$j=1$ {\bfseries to} $\tau$}
%        \STATE $\hat{y}_j^{\rm Bayes} \gets \x_j^\top\beta_{\rm Bayes}$, \; $\hat{y}_j^{\rm MAP} \gets \x_j^\top\beta_{\rm MAP}$
%    \ENDFOR
%    \OUTPUT $\curly{\hat{y}^{\rm Bayes}_j}_{j\in\squarebrack{\tau}}$, $\curly{\hat{y}^{\rm MAP}_j}_{j\in\squarebrack{\tau}}$
%\end{algorithmic}
%\end{algorithm}




% \begin{itemize}
%     \item (Subspace estimation) Partition the meta-dataset such that the first set $\Dcal_1$ satisfies $nt = \Omega \round{  d \cdot \min \curly{ \eps^{-6} p_{\min}^{-2} , \eps^{-2} \lambda_{\min}^{-2} \rho^4 } \cdot \log^3(nd/\delta)}$, and $t<d$.
    
%     Use this for subspace estimation which will be good up-to $\ell_2$ error $\eps\rho$ with probability at least $1-\delta$. To proceed, we just require this $\eps<\nicefrac{\Delta}{4\rho}$.
%     \item
%     \begin{itemize}
%         \item (Clustering) The second set $\Dcal_2$ contains $n$ tasks each with $\Omega\round{\log({n}/{\tilde\delta})}$ batches of samples for some $\tilde\delta\in\round{0,1}$, with each batch having $t = \Omega\round{\rho^2\Delta^{-2}\sqrt{k}}$ samples. Cluster these $n$ tasks by computing
%         \[
%         H_{i,j}^{(2l)}= \round{\hat\beta_i^{(2l)} - \hat\beta_j^{(2l)}}^\top\U \U^\top\round{\hat\beta_i^{(2l+1)} - \hat\beta_j^{(2l+1)}},
%         \]
%         for every batch taking their medians and thresholding,
%         \item (Initial parameter estimation) To get $\tilde\eps$ good estimates of $\w_i, p_i$ and $r_i^2$ for all $i\in\squarebrack{k}$ with probability at least $1-\tilde\delta$, take fresh $t$ more samples from the tasks in $\Dcal_2$ which needs to satisfy $n = \Omega\round{\frac{  \,k \log(k/\tilde\delta)}{t\; p_{\rm min}\tilde\eps^2}+ \frac{\log(k/\tilde\delta)}{p_{\rm min}^2}}$ according to Lemma~\ref{lem:distance}.
        
%         $\tilde\eps$ needs to be less than $\nicefrac{\Delta}{\rho}$ to proceed.
%     \end{itemize}
%     \item
%     \begin{itemize}
%         \item (Classification) Given a new task with $t_{\out}$ samples $\curly{\x_j,y_j}_{j\in\squarebrack{t_{\out}}}$, with the estimate of $\hat\w_i$, $\hat{r}_i\ \forall\ i\in\squarebrack{k}$ obtained in the previous step, compute
%         \[
%         \hat{l}_i := -\sumj{1}{t_{\out}} \frac{\round{y_j-\x_j^\top\hat\w_i}^2}{2\hat{r}_i^2} + t_{\out} \log\inv{\hat{r}_i}
%         \]
%         for all $i\in\squarebrack{k}$, and take the $\argmax$ over $i$ to classify. With probability $1-\delta$, the classification is correct if $\enorm{\hat{\w}_i-\w_i} \le  \Delta/10$,  $s_i^2+\esqnorm{\hat{\w}_i-\w_i}\le (1+\Delta^2/50\rho^2)\hat{r}_i^2$, $s_i^2+\Delta^2/2\rho^2 \ge (1+\Delta^2/5\rho^2)\hat{r}_i^2$ for all $i\in\squarebrack{k}$, and $t_{\out}\ge \Theta\round{\rho^4\log (k/\delta)/\Delta^4}$.
%         \item (Refined parameter estimation) If the above conditions are met and if we classify $n$ tasks from $\Dcal_3$ such that
%         \[
%         n = \Omega\round{\frac{  \,d +\log^2(k/\delta)}{tp_{\rm min}\eps^2 }+\frac{  \log(k/\delta)}{p^2_{\rm min} }},
%         \]
%         we can compute $\eps$ good estimates of $\w_i$, $p_i$ and $s_i^2$ for all $i\in\squarebrack{k}$, where $\hat{\w}_i$ is the regression estimate of all the examples in the $i$-th cluster, $\hat{p}_i$ is the empirical estimator of multinomial random variable, and $\hat{s}_i^2 := \round{n\hat{p}_it-d}^{-1}\sum_{j=1}^{n\hat{p}_it}\round{y_j-\hat\w_i^\top \x_j}^2$ for all $i\in\squarebrack{k}$.
%     \end{itemize}
%     \item (Prediction) Given a new task for prediction, we use the MAP/mean of posterior to predict $y$.
% \end{itemize}











==> Meta-Learning Linear Regression_ k-Mixture/algorithm.tex <==
\section{Algorithm} 
\label{sec:algorithm}

We propose a novel  spectral approach (Algorithm~\ref{alg:estimate}) to solve the meta-learning linear regression,   
 consisting of three sub-algorithms: \textit{subspace estimation}, \textit{clustering}, and \textit{classification}.
These sub-algorithms require different types of tasks, depending on how many labelled examples are available. 
 
Clustering  requires 
{\em heay tasks}, where each task is associated with  many labelled examples, but we need a smaller number of such tasks. 
On the other hand, 
for subspace estimation and classification, {\em light tasks} 
are sufficient, where each task is associated with a few labelled examples. However, we need a large number of such tasks. 
In this section, we present the  intuition behind our algorithm design, and the types of tasks required. Precisely analyzing these requirements is the main contribution of this paper, to be presented in Section~\ref{sec:main}. 




\subsection{Intuitions behind the algorithm design}

%We learn the subspace of the true parameters $\w_i$'s using the light tasks and perform clustering of the heavy tasks on that subspace. This provides estimates of the $\w_i$'s, which we use subsequently for classifying the remaining light tasks. As light tasks are abundant, we can get accurate estimates of the meta-parameters. These are used as priors on newly arriving tasks for prediction. 
We give a sketch of the algorithm below.   
Each step of meta-learning is spelled out in full detail in Section~\ref{sec:algorithm_detail}. 
This provides an estimated meta-parameter  $\hat{\theta}=\big(\hat{\W},\; \hat{\s},\; \hat{\p}\big)$.  
When a new task arrives, this can be readily applied to  solve for %the MAP estimation in \eqref{eq:learn_MAP} and Bayes optimal estimation in \eqref{eq:learn_Bayes}. 
prediction, as defined in Definition~\ref{def:predictor}.



\begin{algorithm}[h]
   \caption{}
   \label{alg:estimate}
\medskip
{\bf Meta-learning}
\begin{enumerate}
    \item {\em Subspace estimation.}~Compute subspace $\U$ which approximates ${\rm span}\curly{\w_1,\ldots, \w_k}$, with singular value decomposition. %\Raghav{$\U$ has been used throughout. Should we change it? we don't want to introduce $\U$ yet. Sure.}% using light tasks. 
    %, and project the data onto the subspace $\hat{\U}$.
    \item {\em Clustering.}~Project the heavy tasks onto the subspace of $\U$, perform distance-based $k$ clustering, and estimate $\tilde{\w}_i$ for each cluster.
    %of the heavy tasks in the $k$-dimensional subspace, and estimate $\hat{\w}_i$ for each cluster.
    \item {\em Classification.}~Perform likelihood-based classification of the light tasks using $\tilde{\w}_i$ estimated from the \textit{Clustering} step, and compute the more refined estimates $(\hat{\w}_i, \hat{s}_i, \hat{p}_i)$ of $(\w_i, s_i, p_i)$ for $i\in [k]$.
\end{enumerate}

{\bf Prediction}
\begin{enumerate}
    \item[4.] {\em Prediction.}~Perform MAP or Bayes optimal prediction using the estimated meta-parameter as a prior.
\end{enumerate}
\end{algorithm}





{\bf Subspace estimation.}  
The subspace spanned by the regression vectors, ${\rm span}\{\w_1,\ldots, \w_k\}$, can be easily estimated using data from the (possibly) light tasks with only $t_i \ge 2$. Using any two independent examples from the same task $(\x_{i,1}, y_{i,1}), (\x_{i,2}, y_{i,2})$, it holds that $\E{y_{i,1}y_{i,2}\x_{i,1}\x_{i,2}^\top} = \sum_{j=1}^k p_j \w_j\w_j^\top$. 
With a total of $\Omega(d \log d)$ such examples, the matrix $\sum_{j=1}^k p_j \w_j\w_j^\top$ can be accurately estimated under spectral norm, and so is the column space ${\rm span}\{\w_1,\ldots, \w_k\}$. We call this step \textit{subspace estimation}.

{\bf Clustering.}
Given an accurate estimation of the subspace ${\rm span}\{\w_1,\ldots, \w_k\}$, we can reduce the problem from a $d$-dimensional to a $k$-dimensional regression problem by  projecting $\x$ onto the subspace of $\U$. Tasks with $t_i=\Omega(k)$ examples can be individually trained as the unknown parameter is now in ${\mathbb R}^k$.
 %if we have $t = \Omega(k)$ examples for each task, we could solve the regression problem for each task independently. 
The fundamental question we address is: \textit{What can we do when $t_i=o(k)$?} 
We propose clustering such light tasks based on their estimates of the regression vector $\beta_i$'s, and jointly solve a single regression problem for each cluster.
 
To this end, we borrow techniques from recent advances in property estimation for linear regression. %The key issue here is how to obtain a good clustering when $t = o(k)$. 
Recently, in the contextual bandit setting, \citet{kong2019sublinear} proposed an estimator for the correlation between the linear regressors between a pair of datasets. Concretely, given two datasets  $\{\x_{1,j}, y_{1,j}\}_{j\in [t]}$ and $\{\x_{2,j}, y_{2,j}\}_{j\in [t]}$ whose true (unknown) regression vectors are $\beta_1$ and $\beta_2$, one can estimate $\esqnorm{\beta_1}$, $\esqnorm{\beta_2}$ and $\beta_1^\top \beta_2$ accurately with $t = \Ocal\big(\sqrt{d}\big)$. We use this technique to estimate  $\esqnorm{\beta_{i_2}-\beta_{i_2}}$, whose value can be used to check if the two tasks are in the same clusters. We cluster the  tasks with $t_i=\Omega\big(\sqrt{k}\big)$ into $k$ disjoint clusters. We call this step \textit{clustering}.

After clustering, resulting estimated $\tilde{\w}_i$'s have two sources of error: the error in the subspace estimation, and the error in the parameter estimation for each cluster. If we cluster more heavy tasks, we can reduce the second error but not the first.
We could increase the samples used in subspace estimation, but there is a more sample efficient way: classification. 
 
{\bf Classification.}
We start the classification step, once each cluster has enough (i.e.~$\Omega(k)$) datapoints to obtain a rough estimation of their corresponding regression vector. In this regime, we have  $\BigO{1}$ error in the estimated $\tilde{\w}_i$'s. This is sufficient for us to add more datapoints to grow each of the clusters. When enough data points are accumulated (i.e.~$\tilde\Omega(d)$ for each cluster), then we can achieve any desired accuracy with this larger set of accurately classified tasks. This separation of the roles of the three sub-algorithms is critical in achieving the tightest sample complexity. 

In contrast to the necessary condition of  $t_i=\Omega\big(\sqrt{k}\big)$ for the clustering step, we show that one can accurately determine which cluster a new task belongs to with only $t_i = \Omega(\log k)$ examples once we have a rough initial estimation $\tilde\W$ of the parameter $\W$. 
We grow the clusters by adding tasks with %$t = \Omega(\log k)$ 
%\Raghav{$\log kn_{L2}$? $\tilde\Omega$?} 
a logarithmic number of examples until we have enough data points per cluster to achieve the desired  accuracy. We call this step \textit{classification}. This concludes our algorithm for the parameter estimation (i.e. meta-learning) phase.

%In the learning phase where a new task is provided with $\tau$ training examples, similar to the \textit{classification} step of our algorithm, we show that $\tau = \Omega(\log(k))$ examples suffices to learn the regression vector accurately.  We give the high level description of our algorithm in the next section.



%In this final step, which we called \textit{classification} step, 
%With $t=1$, no computational efficient way is known to obtain meaningful clusters. 

%Our main algorithm consists of three sub-algorithms: subspace estimation, clustering and classification. 


%\noindent 
%{\bf Algorithm.}
%\noindent 
%\subsection{Sketch of the algorithm}







% We propose first clustering the users with a spectral algorithm and then estimating the parameters for each cluster.  

\iffalse
Precisely, for each $i\in [n]$, we define
\begin{align*}
\hat\beta_i^{(1)} = \left(\frac{1}{t} \sum_{j=1}^{t}y_{i,j}\x_{i,j}\right), ~~~ \hat\beta_i^{(2)} =  \left(\frac{1}{t} \sum_{j=t+1}^{2t}y_{i,j}\x_{i,j}\right).
\end{align*}

Define our estimator $\hat\M \in \mathbb{R}^{d \times d}$ to be matrix 
\[
\hat\M \;\coloneqq\;
\frac{1}{2n}\sum_{i=1}^n \round{\hat\beta_i^{(1)}\hat\beta_i^{(2)\top} + \hat\beta_i^{(2)}\hat\beta_i^{(1)\top}},
\]
and 
$\M\coloneqq\sum_{j=1}^k p_j \w_j\w_j^\top$ to be its expectation. %\Sewoong{Does projection onto PSD cone change the expectation? Perhaps we should remove the projection step.} \Weihao{Nevermind, we don't need the projection step.}
\Raghav{I think it will be great if we can write something about the choice of $\hat{\M}$ in contrast to what Vempala and Wang use. May be some reference of the high level technical advantage.}
\fi


==> Meta-Learning Linear Regression_ k-Mixture/formulation.tex <==
\section{Problem formulation and notations} 
\label{sec:model} 

There are two perspectives
on approaching meta-learning: 
 optimization based 
 \cite{LZC17,BHT18,ZWL18,ZSK19,RFK19}, and probabilistic \cite{grant2018recasting,FXL18,KYD18,HSP18}. 
 Our approach is motivated by the probabilistic view and we present a brief preliminary in Section~\ref{sec:metalearning}. 
 %, optimization based methods can also be derived from the probabilistic perspective of \cite{grant2018recasting}. 
%In Section~\ref{sec:metalearning}, we present a brief preliminary on the  probabilistic view of meta-learning. 
%, and refer to~\cite{grant2018recasting} for a comprehensive introduction.
In Section~\ref{sec:linear}, we  present a simple but  
 canonical scenario where the tasks are linear regressions, which is the focus of this paper. 

\subsection{Review of probabilistic view on meta-learning}
\label{sec:metalearning}


A standard meta-training for few-shot supervised learning assumes that  
we are given a collection of $n$ meta-training tasks $\{{\cal T}_i\}_{i=1}^n$  drawn from some distribution $\P\round{{\cal T}}$.  
Each task is associated with a  dataset of size $t_i$, collectively denoted as a {\em meta-training dataset} 
${\cal D}_{\rm  meta\text{-} train}=\curly{ \{(\x_{i,j},y_{i,j})\in \Rd{d} \times \Rd{}\}_{j\in[t_i]} }_{i\in[n]}$. 
Exploiting  some structural similarities 
in $\P{({\cal T})}$, the goal is to train 
a model for a new task ${\cal T}^{\rm new}$, coming from $\P\round{{\cal T}}$, from a small  amount of {\em training dataset} ${\cal D}=\curly{(\x^{\rm new}_j,y^{\rm new}_j)}_{j\in[\tau]}$. 


%We use $\w_1,\ldots, \w_k\in \Rd{d}$ to denote . Let $\Wcal$ be the uniform distribution supported on $\curly{\w_1,\ldots, \w_k}$. Assuming that for each %person $i\in [n]$, $\beta_i\sim \Wcal$ and $\x_{i,j}\sim \Ncal\round{\zero,\I_d}$, $y_{i,j} = \beta_i^\top \x_{i,j}+\epsilon_{i,j}$ where $\eps_{i,j}\sim \Ncal(0, \sigma_i^2)$ for all $j\in [t]$. 
Each  task ${\cal T}_i$ is associated with 
a {\em model parameter} $\phi_i$, where the meta-training data is independently drawn from: $(\x_{i,j},y_{i,j}) \sim {\mathbb P}_{\phi_i}(y | \x) {\mathbb P}(\x)$ for all $j\in[t_i]$. 
The prior distribution of the 
tasks, and hence the model parameters, is 
fully characterized by a 
{\em meta-parameter} $\theta$ such that $\phi_i \sim {\mathbb P}_{\theta}(\phi)$. 


Following the definition from \cite{grant2018recasting}, the {\em meta-learning problem} is defined as estimating the most likely meta-parameter given meta-training data by solving 
\begin{eqnarray}
    \theta^* \;\; \in \;\; \argmax_\theta \;\;\log \,\P{ ( \theta\,|\, {\cal D}_{\rm meta\text{-}data} )}\;,
    \label{eq:metalearning}
\end{eqnarray}
which is a special case of empirical Bayes methods for learning the prior distribution from data \cite{carlin2010bayes}. 
Once meta-learning is done, the model parameter of a newly arriving task can be 
estimated by a Maximum a Posteriori (MAP) estimator: 
\begin{eqnarray}
   \hat{\phi} \;\in\; \argmax_\phi
   \;\; \log \,\P{( \phi  \,|\, {\cal D}, \theta^*)}\;,
   \label{eq:learn_MAP}
\end{eqnarray}
or a Bayes optimal estimator:  
\begin{eqnarray}
   \hat{\phi} \;\in\; \argmin_\phi
   \;\; {\mathbb E}_{\phi'\sim \P{( \phi'  \,|\, {\cal D}, \theta^*)}} 
   [ \,\ell(\phi,\phi') \, ] \;,
   \label{eq:learn_Bayes}
\end{eqnarray}
for a choice of a loss function $\ell$. 
This estimated parameter is then used for predicting the label of a new data point $\x$ in task ${\cal T}^{\rm new}$ as 
\begin{eqnarray}
    \hat{y}\;\;\in\;\; \argmax_{y} \;\; {\mathbb P}_{\hat\phi}(y|\x) \;.
    \label{eq:predict}
\end{eqnarray}

\paragraph{General notations.} %We define a few notations for some mathematical objects we shall use. 
We define $\squarebrack{n}\coloneqq\curly{1,\ldots,n}\ \forall\ n\in\Natural$; $\norm{\x}_{p} \coloneqq \round{\sum_{x\in\x}\abs{x}^p}^{1/p}$ as the standard $\ell_p$-norm; and $B_{p,k}(\muvec,r) \coloneqq \curly{\x\in\Rd{k} \mid \norm{\x-\muvec}_{p} = r}$. 
%\forall\ p\geq 1$, $k\in\Natural$, $\muvec\in\Rd{k}$, and $r\in\R_+$;
$\Ncal\round{\muvec,\SIGMA}$ denotes the multivariate normal distribution with mean $\muvec\in\Rd{d}$ and covariance $\SIGMA\in\Rd{d\times d}$, and  $\indicator{E}$ denotes the indicator  of an event $E$.


% ------------------------------


\subsection{Linear regression with a discrete prior} 
\label{sec:linear}
In general, the meta-learning problem of \eqref{eq:metalearning} is computationally intractable and no statistical guarantees are known.  
To investigate the trade-offs involved, we assume  a simple but canonical scenario where the tasks are linear regressions: 
\begin{eqnarray}
     \x_{i,j}\sim\Pcal_{\x}\;,\;\;\;\;\; 
    y_{i,j} = \beta_i^\top \x_{i,j}+\epsilon_{i,j}\;,  
    \label{eq:model}
\end{eqnarray}
for the $i$-th task and $j$-th example. 
Each task is associated with a model parameter $\phi_i=\round{\beta_i\in{\mathbb R}^d, \sigma_i \in {\mathbb R}_+}$. % for all $i\in\squarebrack{n}$.
The noise $\eps_{i,j}$ is i.i.d.~as~$\eps_{i,j}\sim \Pcal_{\eps_i}$, and $\Pcal_{\eps_i}$ is a centered sub-Gaussian distribution with parameter $\sigma_i^2$. Without loss of generality, we assume that $\Pcal_{\x}$ is an isotropic (i.e. $\E{\x_{i,j}\x_{i,j}^\top} = \I_d$) centered sub-Gaussian distribution. If $\Pcal_{\x}$ is not isotropic, we assume there are large number of $\x_{i,j}$'s for whitening such that $\Pcal_{\x}$ is sufficiently close to isotropic.
% with second moment $\I_d$. 


We do not make any assumption on the prior of $\phi_i$'s 
other than that they come from a discrete distribution of a support size $k$. Concretely, the meta-parameter 
$\theta=\round{\W\in{\mathbb R}^{d\times k},\; \s\in{\mathbb R}^{k}_+,\; \p\in{\mathbb R}^{k}_+\cap B_{1,k}(\zero,1)}$
defines a discrete prior (which is also known as mixture of  linear experts \cite{CL13}) on $\phi_i$'s, 
where 
$\W=[\w_1,\ldots, \w_k] $ 
are the $k$ candidate model parameters, and  
$\s=[s_1,\ldots,s_k] $ are the $k$ candidate noise parameters. The $i$-th task is randomly chosen from one of the $k$ components from  distribution $\p$, denoted by $z_i\sim{\rm multinomial}(\p)$. The  training data is independently drawn from~\eqref{eq:model} for each $j\in[t_i]$  with $\beta_i=\w_{z_i}$ and $\sigma_i = s_{z_i}$.
%in the $(k-1)$-dimensional simplex. The  $t$ labeled data points are then drawn from 

 We want to characterize 
 the sample complexity of this meta-learning. This depends on how complex the 
 ground truths prior $\theta$ is. 
 This can be measured by the number of components $k$, the separation between the parameters $\W$, the minimum mixing probability $p_{\rm min}$, and the minimum positive eigen-value $\lambda_{\rm min}$ of the matrix $\sum_{j=1}^{k}p_j\w_j\w_j^\top$.

 
% which can be used directly to solve~\eqref{eq:learn}  as 
%\begin{eqnarray}
%\hat{i} &\coloneqq\; \argmax\limits_{i\in[k]} \inv{2\hat{s}_i^2}\sum\limits_{j\in[\tau]}-\round{\hat{\w}_i^\top\x^{\rm new}_j - y_j^{\rm new}}^2\nonumber\\
%&\qquad\qquad\qquad\qquad\qquad+\tau\log \frac{1}{\hat{s}_i} +\log\round{\hat{p}_i}, 
%\label{eq:learnlinear}
%\end{eqnarray}
%and let $\hat{\beta}=\hat{\w}_{\hat{i}}$ where $\hat{i}$ is the optimizer of the maximization in~\eqref{eq:learnlinear}. \Raghav{Should we also talk about Bayes optimal estimator here?} The prediction in 
%\eqref{eq:predict} simplifies to 
%$\hat{y} = \hat\beta^\top\x$, and is evaluated on 
%the prediction error:
%\begin{eqnarray}
%    \Exp{\round{\x^{\rm test},y^{\rm test}}}{\, \round{ \hat{\beta}^\top\x^{\rm test} - y^{\rm test} }^2 \,}\;,
%    \label{eq:performance}
%\end{eqnarray}
%where the test example $\round{\x^{\rm test},y^{\rm test}}$ is drawn from \eqref{eq:model} with 
%$\beta_i=\w_{z^{\rm new}}$ and $\sigma_i=s_{z^{\rm new}}$. 


{\bf Notations.} 
% $\rho_i^2 \coloneqq \Var{y_{i,1}|z_i} = s_{z_i}^2+\esqnorm{\w_{z_i}}$
We define $\rho_i \coloneqq \sqrt{s_{z_i}^2+\esqnorm{\w_{z_i}}}$ as the sub-Gaussian norm of a label $y_{i,j}$ in the $i$-th task, and $\rho^2 \coloneqq \max_{i} \rho_i^2$. %\Sewoong{variance and sub-Gaussian parameter is not the same.}
Without loss of generality, we assume $\rho=1$, which can be always  achieved by scaling the meta-parameters appropriately. We also define $p_{\rm min}\coloneqq\min_{j\in[k]}p_j$, and $\Delta\coloneqq \min_{i,j\in\squarebrack{k}, i\neq j}\enorm{\w_i-\w_j}$ and assume $p_{\rm min}, \Delta>0$. $\omega\in\R_+$ is such that two $n\times n$ matrices can be multiplied in $\BigO{n^\omega}$ time.
 %Without loss of generality, we assume $\enorm{\w_1}\geq \enorm{\w_2} \geq \cdots \geq \enorm{\w_k}$.\Raghav{Do we need this ordering anywhere?}

==> Meta-Learning Linear Regression_ k-Mixture/intro.tex <==
\section{Introduction}
\label{sec:intro} 

Recent advances in machine learning highlight successes on a small set  of tasks where a large number of labeled examples have been collected and exploited. These include image classification with 1.2 million labeled examples~\cite{deng2009imagenet} and French-English machine translation with 40 million paired sentences~\cite{bojar2014findings}. For common tasks, however, collecting clean labels is costly, as they require human expertise (as in medical imaging) or  physical interactions (as in robotics), for example. Thus collected real-world datasets follow a long-tailed distribution, in which a dominant set of tasks only have a small number of training examples~\cite{wang2017learning}. 

Inspired by human ingenuity in quickly solving novel problems by leveraging prior experience,  {\em meta-learning}  approaches aim to jointly learn from past experience to quickly adapt to new tasks with little available data \cite{Sch87,TP12}. This has had a significant impact in few-shot supervised learning, where each task is associated with only a few training examples. By leveraging structural similarities among those tasks, one can achieve accuracy far greater than what can be achieved for each task in isolation \cite{FAL17,RL16,KZS15,OLL18,triantafillou2019meta,rusu2018meta}. 
%This is critical in democratizing machine learning  %where small data tasks can help each other in achieving the accuracy of big data tasks. 
The success of such approaches hinges on the following fundamental question: When can we jointly train small data tasks to achieve the accuracy of  large data tasks? 



% data has long tail - cannot be learned in isolation, remedy is meta-learning: leveraging past experience to make predictions on new tasks more accurate. empirical successes.  

% fundamental question: when can it compaensate for ? how many small data is equivalent to alrge data? 


% we address this in a canonical setting of linear regressions. regression parameter w_i, p_i, for some finite set of k.  

We investigate this trade-off under a canonical scenario where the tasks are linear regressions in $d$-dimensions and the regression parameters are drawn i.i.d.~from a discrete set of a support size $k$. 
Although widely studied, existing literature addresses the scenario  where 
 %each task only has one example (known as mixed linear regression) and where 
all tasks have the same fixed number of examples. %(known as multi-task learning). 
We defer formal comparisons to Section~\ref{sec:related}. 

On one extreme, when large training data of sample size $\Omega(d)$ is available, each task can easily be learned in isolation; here, $\Omega(k\log k)$ such tasks are sufficient to learn all $k$ regression parameters. This is illustrated by a solid circle in Figure~\ref{fig:intro}. On the other extreme, when each task has only one example, existing approaches require exponentially many tasks (see Table~\ref{tab:related}). This is illustrated by a solid square.

Several aspects of  few-shot supervised learning makes training linear models  challenging. The number of training examples varies significantly across tasks, all of which are significantly smaller than the dimension of the data $d$. The number of tasks are also limited, which  restricts 
any algorithm with exponential sample complexity. 
An example distribution of 
such heterogeneous tasks is illustrated in Figure~\ref{fig:intro} with a bar graph in blue, where both the solid circle and square are far outside of the regime covered by the typical  distribution of tasks. 

%should be close to $kd$, which is the information theoretic lower bound on how many examples are necessary to learn the $k$ linear models each in $d$ dimensions. 

\begin{figure}[ht] 
\begin{center} 
\centerline{\includegraphics[width=.5\columnwidth]{figure}}
\caption{ 
Realistic pool of meta-learning tasks do not include large data tasks (circle) or extremely large number of small data tasks (square), where existing approaches achieve high accuracy. 
The horizontal axis denotes the number of examples $t$ per task, and the vertical axis denotes the number of tasks in the pool that have at least $t$ examples. The proposed approach succeeds whenever any point in the light (green) region, and any point in the heavy (yellow) region are both covered by the blue bar graph, as is in this example. The blue graph summarizes the pool of tasks in hand, illustrating the cumulative count of tasks with more than $t$ examples.
We ignore constants and ${\rm poly}\log$ factors.}
\label{fig:intro} 
\end{center} 
\end{figure} 

In this data scarce regime,  we show that we can still efficiently achieve any desired accuracy in estimating the meta-parameters defining the meta-learning problem. This is shown in the informal version of our main result in Corollary~\ref{cor:main}. As long as we have enough number of {\em light tasks} each with $t_L=\tilde\Omega(1)$ examples, we can achieve any accuracy with the help of a small number of {\em heavy tasks} each with $t_H= \tilde{\Omega}(\sqrt{k})$ examples. We only require the total number of examples that we have jointly across all light tasks to be of order $t_Ln_L=\tilde\Omega(dk^2)$; the number of light tasks $n_L$ and the number of examples per task $t_L$ trade off gracefully. This is illustrated by the green region in Figure~\ref{fig:intro}. Further, we only need a small number of heavy tasks  with $t_Hn_H=\tilde\Omega(k^{3/2})$, shown in the yellow region. As long as the cumulative count of tasks in blue graph intersects with the light (green) and heavy (yellow) regions, we can recover the meta-parameters accurately. 

%\Sewoong{
%Kaggle's diabetic retinopathy detection dataset 35k labeled images
%Adaptive epilepsy treatment with RL, Guez et al. 08 <1hour data 
%Learning for robotic manipulation Finn et al. '16 <15min data
%}



%{\bf Meta-learning.}\cite{FAL17,LZC17,FXL18,BHT18,ZWL18,ZSK19}Computational and memory burden of evaluating the gradient for the inner loop optimization was solved \cite{RFK19} by making the inner loop implicit. 

%There is a fundamental question of interest: How large $n$ needs to be, such that given a new person with $t_{test}$ samples our algorithm is close to the optimal algorithm that knows $\Wcal$? \Sewoong{perhaps we should rephrase this.}




\begin{corollary}[Special case of Theorem~\ref{thm:main_reg_est}, informal]\hfill
\label{cor:main}
%\begin{enumerate}
%\item Suppose $\Delta = \Omega(1)$, and $p_{\rm min} = \Omega(1/k)$. 
Given two batch of samples, the first batch with
\[
t_L = \tilde\Omega(1)\;,\;t_Ln_L = \tilde\Omega\round{dk^2},
\]
and the second batch with 
\[
t_H = \tilde\Omega\big(\sqrt{k}\big)\;,\;t_Hn_H = \tilde\Omega\big(k^{2}\big),
\]
Algorithm~\ref{alg:estimate} estimates the meta-parameters up to any desired accuracy of $\BigO{1}$ with a high probability, under a certain assumptions on the meta-parameters.
%\begin{align*}
%\enorm{\hat{\w}_i-\w_i} &\le \eps s_i\; , \\ 
%\abs{\hat{s}_i^2-s_i^2}&\le  \frac{\eps}{\sqrt{d}}s_i^2\; ,\quad\text{and}\\
%\abs{\hat{p}_i-p_i} &\le \frac{\eps}{\sqrt{d}} p_i.
%\end{align*}
%\item
%Given a new task $\cal T^{\rm new}$ with $\tau\ge \Theta\round{\log (k/\delta)}$ samples $\mathcal{D} = \{ \x_i,y_i\}_{i=1}^\tau$. 
%Then, the MAP/posterior mean estimator $\hat{\beta}$ using the estimated parameters approximates the true regression vector $\beta^{\rm new}$ with expected $\ell_2$ error bounded as
%\begin{align*}
%&\mathbb{E}_{\cal T^{\rm new} \sim \P{(\cal T)}}\mathbb{E}_{\cal D \sim \cal T^{\rm new}}\squarebrack{\esqnorm{\hat{\beta}({\cal D})-\beta^{\rm new}}}\le \delta+\eps^2
%\end{align*}
%\end{enumerate}
\end{corollary}

We design a novel spectral approach inspired by \cite{vempala2004spectral} that first learns a subspace using the light tasks, and then clusters the heavy tasks in the projected space. To get the desired tight bound on the sample complexity, we improve upon a perturbation bound from \cite{li2018learning}, and borrow techniques from recent advances in property testing in \cite{kong2019sublinear}. 


%\Sewoong{Meta-learning addresses a challenging scenario of a data poor regime where $(a)$ we might have a large number of tasks $n$, but each task has only a small number $t\ll d$ of  labelled examples; and $(b)$ the model for a new task needs to be learned from an even smaller  $\tau \ll t$ number of labelled examples.}








==> Meta-Learning Linear Regression_ k-Mixture/macro.tex <==
% Weihao's macros 
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\ov}{\overline}
\newcommand{\eps}{\epsilon}
\newcommand{\N}{\mathcal{N}}
\newcommand{\R}{\mathbb{R}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\RHS}{\mathrm{RHS}}
\newcommand{\LHS}{\mathrm{LHS}}
\renewcommand{\d}{\mathrm{d}}
\renewcommand{\i}{\mathbf{i}}
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\renewcommand{\varepsilon}{\epsilon}
\renewcommand{\tilde}{\wt}
\renewcommand{\hat}{\wh}
\renewcommand{\eps}{\epsilon}
\newcommand{\diag}{\textrm{diag}}
\renewcommand{\d}{\mathrm{d}}

\newtheorem{propo}{Proposition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{definition}[propo]{Definition}
%\newtheorem{coro}[propo]{Corollary}
\newtheorem{thm}[propo]{Theorem}
\newtheorem{asmp}{Assumption}
%\newtheorem{theorem}[propo]{Theorem}
%\newtheorem{conj}[propo]{Conjecture}
%\newtheorem{fact}[propo]{Fact}
%\newtheorem{remark}[propo]{Remark}
%\newtheorem{claim}[propo]{Claim}

% Raghav's macros
% theorem styles
% \theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{notation}[theorem]{Notation}
% \newtheorem{proof}[theorem]{Proof}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{example}[theorem]{Example}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{open}[theorem]{Open Problem}
\newtheorem{hypothesis}[theorem]{Hypothesis}
\newtheorem{question}[theorem]{Question}

% brackets
\newcommand{\round}[1]{\left( #1 \right)}
\newcommand{\curly}[1]{\left\lbrace #1 \right\rbrace}
\newcommand{\squarebrack}[1]{\left\lbrack #1 \right\rbrack}

% sums
\newcommand{\sumi}[2]{\sum\limits_{i=#1}^{#2}}
\newcommand{\sumj}[2]{\sum\limits_{j=#1}^{#2}}
\newcommand{\sumk}[2]{\sum\limits_{k=#1}^{#2}}
\newcommand{\sump}[2]{\sum\limits_{p=#1}^{#2}}
\newcommand{\suml}[2]{\sum\limits_{l=#1}^{#2}}
\newcommand{\sumn}[2]{\sum\limits_{n=#1}^{#2}}
\newcommand{\summ}[2]{\sum\limits_{m=#1}^{#2}}
\newcommand{\sumt}[2]{\sum\limits_{t=#1}^{#2}}

\newcommand{\Sum}{\sum_{i = 1}^{n}}
\newcommand{\Sumi}[1]{\sum\limits_{i = 1}^{#1}}
\newcommand{\Sumt}[1]{\sum\limits_{t = 1}^{#1}}

% norms
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\esqnorm}[1]{\left\lVert#1\right\rVert_2^2}
\newcommand{\enorm}[1]{\left\lVert#1\right\rVert_2}
\newcommand{\infnorm}[1]{\left\lVert#1\right\rVert_\infty}
\newcommand{\opnorm}[1]{\left\lVert#1\right\rVert_\text{op}}
\newcommand{\normF}[1]{\left\lVert#1\right\rVert_{\text{F}}}
\newcommand{\inner}[1]{\left\langle#1\right\rangle}
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil}
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor}

% bold numbers
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}

% bold small english vectors
\newcommand{\avec}{\mathbf{a}}
\newcommand{\bvec}{\mathbf{b}}
\newcommand{\cvec}{\mathbf{c}}
\newcommand{\dvec}{\mathbf{d}}
\newcommand{\e}{\mathbf{e}}
\newcommand{\f}{\mathbf{f}}
\newcommand{\g}{\mathbf{g}}
\newcommand{\h}{\mathbf{h}}
\newcommand{\ivec}{\mathbf{i}}
\newcommand{\jvec}{\mathbf{j}}
\newcommand{\kvec}{\mathbf{k}}
\newcommand{\lvec}{\mathbf{l}}
\newcommand{\m}{\mathbf{m}}
\newcommand{\n}{\mathbf{n}}
\newcommand{\ovec}{\mathbf{o}}
\newcommand{\p}{\mathbf{p}}
\newcommand{\q}{\mathbf{q}}
\newcommand{\rvec}{\mathbf{r}}
\newcommand{\s}{\mathbf{s}}
\newcommand{\tvec}{\mathbf{t}}
\newcommand{\uvec}{\mathbf{u}}
\newcommand{\vvec}{\mathbf{v}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\x}{\mathbf{x}}

\newcommand{\y}{\mathbf{y}}
\newcommand{\z}{\mathbf{z}}

% bold capital english matrices
\newcommand{\A}{\mathbf{A}}
\newcommand{\B}{\mathbf{B}}
% \newcommand{\C}{\mathbf{C}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\Emat}{\mathbf{E}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\G}{\mathbf{G}}
\newcommand{\Hmat}{\mathbf{H}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\J}{\mathbf{J}}
\newcommand{\K}{\mathbf{K}}
\newcommand{\Lmat}{\mathbf{L}}
\newcommand{\M}{\mathbf{M}}
% \newcommand{\N}{\mathbf{N}}
\newcommand{\Omat}{\mathbf{O}}
\newcommand{\Pmat}{\mathbf{P}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\Rmat}{\mathbf{R}}
\newcommand{\Smat}{\mathbf{S}}
% \newcommand{\T}{\mathbf{T}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\W}{\mathbf{W}}
\newcommand{\X}{\mathbf{X}}
\newcommand{\Y}{\mathbf{Y}}
\newcommand{\Z}{\mathbf{Z}}

% bold capital greek matrices
\newcommand{\SIGMA}{\mathbf{\Sigma}}
\newcommand{\LAMBDA}{\mathbf{\Lambda}}

% capital mathcal
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

% small greek bold vectors
\newcommand{\alphavec}{\boldsymbol{\alpha}}
\newcommand{\betavec}{\boldsymbol{\beta}}
\newcommand{\gammavec}{\boldsymbol{\gamma}}
\newcommand{\deltavec}{\boldsymbol{\delta}}
\newcommand{\epsvec}{\boldsymbol{\epsilon}}
\newcommand{\etavec}{\boldsymbol{\eta}}
\newcommand{\nuvec}{\boldsymbol{\nu}}
\newcommand{\tauvec}{\boldsymbol{\tau}}
\newcommand{\rhovec}{\boldsymbol{\rho}}
\newcommand{\lmbda}{\boldsymbol{\lambda}}
\newcommand{\muvec}{\boldsymbol{\mu}}
\newcommand{\thetavec}{\boldsymbol{\theta}}

% complexity notations
\newcommand{\BigO}[1]{\mathcal{O}\round{#1}}
\newcommand{\BigOmega}[1]{\Omega\round{#1}}

% Set notations
% \newcommand{\R}{\mathbb{R}}
\newcommand{\Rd}[1]{\mathbb{R}^{#1}}
\newcommand{\Natural}{\mathbb{N}}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Integer}{\mathbb{Z}}
\newcommand{\Rational}{\mathbb{Q}}

% Probability
\DeclareMathOperator*{\myE}{\mathbb{E}}
\newcommand{\E}[1]{\myE\squarebrack{#1}}
\newcommand{\Exp}[2]{\myE_{#1}\squarebrack{#2}}
\newcommand{\Prob}[1]{\mathbb{P}\squarebrack{#1}}
\newcommand{\Var}[1]{\mathrm{Var}\squarebrack{#1}}

% math shortcuts
\newcommand{\inv}[1]{\frac{1}{#1}}
\newcommand{\indicator}[1]{\mathbbm{1}\curly{#1}}
\newcommand{\Tr}[1]{\text{Tr}\squarebrack{#1}}

% others
\newcommand{\BOX}[1]{\fbox{\parbox{\linewidth}{\centering#1}}}
\newcommand{\textequal}[1]{\stackrel{#1}{=}}
\newcommand{\textleq}[1]{\stackrel{#1}{\leq}}
\newcommand{\textgeq}[1]{\stackrel{#1}{\geq}}

% calculus
\newcommand{\dd}[2]{\frac{d #1}{d #2}}
\newcommand{\ddn}[3]{\frac{d^{#1} #2}{d #3^{#1}}}
\newcommand{\dodo}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\dodon}[3]{\frac{\partial^{#1} #2}{\partial {#3}^{#1}}}




==> Meta-Learning Linear Regression_ k-Mixture/main_results.tex <==


\section{Main results}
\label{sec:main}


Suppose we have 
$n_H$ heavy tasks each with at least $t_H$ training examples, and $n_L$ light tasks
each with at least $t_L$ training examples. 
If heavy tasks are  data rich ($t_H\gg d$), we can learn $\W$ straightforwardly from a relatively small number, i.e.~$n_H = \Omega(k \log k)$.
If the light tasks are data rich ($t_L \gg k$), they can be straightforwardly clustered on the projected $k$-dimensional subspace.  
We therefore focus on the  following challenging regime of data scarcity. 


\begin{asmp}
    \label{asmp}
    The heavy dataset ${\cal D}_{H}$ consists of 
    $n_H$ heavy tasks, each with at least $t_H$ samples. 
    The first light dataset ${\cal D}_{L1}$
    consists of $n_{L1}$ light tasks, 
    each with at least $t_{L1}$ samples. 
    The second light dataset ${\cal D}_
    {L2}$
    consists of 
    $n_{L2}$ tasks,
    each with at least $t_{L2}$ samples.
    We assume $t_{L1}, t_{L2}<k, $ and $t_H<d$. 
\end{asmp}

To give  more fine grained analyses on the 
sufficient conditions, 
we assume two types of light tasks are available with potentially differing sizes (Remark~\ref{rem:twotype}). 
In meta-learning step in Algorithm~\ref{alg:estimate},  subspace estimation uses ${\cal D}_{L1}$, 
clustering uses ${\cal D}_H$, and 
classification uses ${\cal D}_{L2}$. 
We provide proofs of the main results  in Appendices~\ref{sec:proof_est},  \ref{sec:proof_pred}, and 
\ref{sec:lb-predict-proof}.


%{\bf implicitly assume $s_i=\BigO{1}$ and keep track of only $\Delta$.} 

% =============================
\subsection{Meta-learning}


We characterize a sufficient condition to
achieve a target accuracy $\epsilon$ in estimating the meta-parameters $\theta=(\W,\s,\p)$. 

\begin{thm}[Meta-learning]\label{thm:main_reg_est}
For any failure probability $\delta \in (0,1)$, and accuracy $\epsilon \in (0,1)$, given three batches of samples under Assumption~\ref{asmp}, meta-learning step of Algorithm~\ref{alg:estimate} estimates the meta-parameters with accuracy 
\begin{align*}
\enorm{\hat{\w}_i-\w_i} &\;\le\; \eps s_i\; , \\ 
\abs{\hat{s}_i^2-s_i^2}&\;\le\;  \frac{\eps}{\sqrt{d}}s_i^2\; ,\quad\text{and}\\
\abs{\hat{p}_i-p_i} &\;\le\; \eps \sqrt{\frac{t_{L2}}{d}}\;p_i\;, 
\end{align*}
with probability at least $1-\delta$, if the following holds. The numbers of tasks satisfy 
\begin{align*}
n_{L1} &= \Omega \round{\frac{d\,\log^3\round{\frac{d}{p_{\rm min}\Delta\delta}}}{t_{L1}} \cdot \min \curly{ \Delta^{-6} p_{\min}^{-2} , \Delta^{-2} \lambda_{\min}^{-2} }  }\;,\\
%\end{align*} 
%number of examples for \textit{subspace estimation}, 
%\begin{eqnarray*}
n_{H} & =\; \Omega\round{\frac{  \, \log(k/\delta)}{t_H\; p_{\rm min}\Delta^2}\round{k+\Delta^{-2}}}\;,\\
%\end{eqnarray*}
%i.i.d. tasks each with 
%\begin{eqnarray*}
n_{L2} & =\; \Omega\round{\frac{  \,d\log^2(k/\delta)}{t_{L2}p_{\rm min}\eps^2 }}\;,
\end{align*}
and the numbers of samples  per task  satisfy 
$t_{L1}\ge 2$, 
 % number of examples for \textit{clustering}, the third batch with 
 $t_{L2} = \Omega\round{\log\round{{kd}/({p_{\rm min}\delta\eps)}}/\Delta^4}$, 
 and $t_H = \Omega\round{\Delta^{-2}\sqrt{k}\log\round{{k}/({p_{\rm min}\Delta\delta})}}$, where $\lambda_{\min}$ is the smallest non-zero eigen value of $\M\coloneqq\sum_{j=1}^k p_j \w_j\w_j^\top \in \mathbb{R}^{d \times d}$. 
%examples for \textit{classification}, . 
\end{thm}

In the following remarks, we explain each of the conditions.  

\begin{remark}[Dependency in ${\cal D}
_{L1}$]
The total number of samples used in subspace estimation is  $n_{L1} t_{L1}$. The sufficient condition scales linearly in $d$ which matches the  information theoretically necessary condition up to logarithmic factors. 
If the  matrix $\M$ is well conditioned, for example when $\w_i$'s are all orthogonal to each other, subspace estimation is easy, and $n_{L1}t_{L1}$ scales as $\Delta^{-2} \lambda_{\min}^{-2}$. Otherwise, the problem gets harder, and we need $\Delta^{-6} p_{\min}^{-2}$ samples.
% \Raghav{The tighter requirement now looks like
% \begin{eqnarray*}
%     n_{L1} &\geq \tilde\Omega\round{\max\curly{\min\curly{\Delta^{-2}\lambda_{\rm min}^{-2},\Delta^{-6} p_{\rm min}^{-2}},dt_{L1}^{-1}\min\curly{\Delta^{-1}\lambda_{\min}^{-1},\Delta^{-3}p_{\rm min}^{-1}}}}
% \end{eqnarray*}
% if $\log(n_{L1}d)\cdot\max\curly{\Delta\lambda_{\rm min},\Delta^3p_{\rm min}}\gtrsim 1$, which in the orthonormal uniform case means $k\lesssim \log(n_{L1}d)$.}\Weihao{Where does this come from?}
Note that in this regime, tensor decomposition approaches often fails to provide any meaningful guarantee (see Table~\ref{tab:related}). In proving this result, 
we improve upon a matrix perturbation bound  in % Lemma~5 of 
\cite{li2018learning} to 
shave off a $k^6$ factor on $n_{L1}$
 (see Lemma~\ref{lem:lemma_5_in_ll18}). 
 
% In an ideal case where, $p_{\rm min}=\Omega(1/k)$, $\Delta=\Omega(1)$, and the $\w_i$'s are well separated, the sufficient condition for subspace estimation is  $n_{L_1}t_{L_1}=\BigO{k^2 d}$. This is a factor of $k$ larger than the information theoretic necessary condition, ...???
 
\end{remark}

\begin{remark}[Dependency in ${\cal D}_H$]
The 
clustering step 
requires 
$t_H =\tilde{\Omega}(\sqrt{k})$, which is necessary for distance-based 
  clustering approaches such as 
  single-linkage clustering. 
  From \cite{kong2018estimating, kong2019sublinear}   we know that it is necessary (and sufficient) 
  to have $t = \Theta(\sqrt{k})$, 
even for a  simpler 
 testing problem between $\beta_1 = \beta_2$ or $\esqnorm{\beta_1-\beta_2}\gg 0$, from 
 two labelled datasets  
 %of data points $\{(\x_{1,i}, y_{1,i})\in{\mathbb R}^{k+1}\}_{i\in [t]}$ and $\{(\x_{2,i}, y_{2,i})\in{\mathbb R}^{k+1}\}_{i\in [t]}$ whose true (unknown) regression vectors are 
 with two linear models $\beta_1$ and $\beta_2$. 
 
 Our clustering step is inspired by \cite{vempala2004spectral} on clustering under Gaussian mixture models, where  
 the algorithm succeeds if  
 $t_H =\tilde\Omega( \Delta^{-2} \sqrt{k} )$. 
 Although a straightforward adaptation  fails, 
 we match the sufficient condition. 
% The key is using the median of estimates to get   Lemma~\ref{lem:distance}. 
 
We only require the  number of heavy samples $n_Ht_H$ to be $\tilde\Omega\round{{k}/{p_{\rm min}}}$  up to logarithmic factors,  
 which is information theoretically necessary.
 %such that the smallest cluster has $n_2t_2p_{\rm min} = \Omega(k)$ samples. This matches the information theoretic lower bound of a  $k$-dimensional regression problem. 
\end{remark}


\begin{remark}[Gain of using two types of light tasks]
\label{rem:twotype}
To get the tightest guarantee, it is necessary to use a different set of light tasks to perform the final estimation step. 
First notice that the first light dataset $\Dcal_{L1}$ does not cover the second light dataset since we need $t_{L2}\ge \Omega(\log (kd))$ which does not need to hold for the first dataset $\Dcal_{L1}$. On the other hand, the second light dataset does not cover the first light dataset in the setting where $\Delta$ or $p_{\rm min}$ is very small. 

%If we use the (previously clustered) heavy tasks, we would need the number of heavy tasks $n_H$ to be at least $\Omega(d/\eps^2)$, which is unnecessarily large.
%If we use the (previously used) light tasks, we would need 
\end{remark}


\begin{remark}[Dependency in ${\cal D}_{L2}$]
Classification and prediction use the same routine to classify the given task. 
 Hence, the $\log k$ requirement in $t_{L2}$ is tight, as it matches  
 our lower bound in  Proposition~\ref{thm:lb-predict}. 
 The extra terms in the $log$ factor come from the union bound over all $n_{L2}$ tasks to make sure all the tasks are correctly classified. It is possible to replace it by $\log(1/\eps)$ by showing that $\eps$ fraction of incorrectly classified tasks does not change the estimation by more than $\eps$. We only require $n_{L2}t_{L2} = \Omega(d/p_{\rm min})$ up to logarithmic factors, 
%ensures that the smallest cluster has at least $d$ samples, 
which is information  theoretically necessary. 
%such that the smallest cluster has $n_3t_3p_{\rm min} = \Omega(d)$ samples since $\Omega(d)$ samples is information theoretically necessary for solving the $d$ dimensional regression problem. 
%The reason for not performing the classification step in the estimated $k$-dimensional subspace  is  
\end{remark}


% =============================
\subsection{Prediction}


Given an estimated meta-parameter 
$\hat\theta=(\hat\W,\hat\s,\hat\p)$, and a new dataset ${\cal D}=\{(\x^{\rm new}_j,y^{\rm new}_j)\}_{j\in[\tau]}$, 
we make predictions on the new task with unknown parameters using two estimators: MAP estimator and Bayes optimal estimator.
%Given a task $\phi^{\rm new} \sim {\mathbb P}_{\theta}$ and its dataset $\cal D \sim {\mathbb P}_{\phi^{\rm new}}$, 

\begin{definition}
\label{def:predictor}
Define the maximum a posterior (\textit{MAP}) estimator as
\[
\hat{\beta}_{\rm MAP}({\cal D}) \coloneqq \hat{\w}_{\hat{i}}\; ,\quad\text{where}\quad \hat{i} \coloneqq \argmax_{i\in\squarebrack{k}} \log \hat{L}_i\;, \text{ and }
\]
\begin{eqnarray*}
\hat{L}_{i} &\coloneqq \exp \round{-\sum\limits_{j=1}^\tau\frac{\round{y^{\rm new}_j-\hat\w_i^\top \x_j^{\rm new}}^2}{2\hat{s}_i^2}-\tau\log\hat{s}_i+\log\hat{p}_i}.
\end{eqnarray*}
Define the posterior mean estimator as
\[
\hat{\beta}_{\rm Bayes}({\cal D}) \coloneqq \frac{\sum_{i=1}^k \hat{L}_i\hat{\w}_{i}}{\sum_{i=1}^k \hat{L}_i}.
\]
\end{definition}

If the true prior, $\{(\w_i,  s_i, p_i)\}_{i\in [k]}$, is known. The posterior mean estimator achieves the smallest expected squared $\ell_2$ error, ${\mathbb E}_{{\cal D},\beta^{\rm new}}\squarebrack{{\esqnorm{{\hat{\beta}({\cal D})-\beta^{\rm new}}}}}$. Hence, we refer to it as 
%In this paper, we also call the posterior mean estimator 
Bayes optimal estimator. The MAP estimator maximizes the probability of exact recovery. 

\begin{thm}[Prediction]\label{thm:main_reg_pred}
Under the hypotheses of Theorem~\ref{thm:main_reg_est} with $\eps\le \min\curly{\Delta/10, \Delta^2\sqrt{d}/50}$, %given a new task $\cal T^{\rm new}$ with 
the expected prediction errors of both the MAP  and Bayes optimal estimators $\hat\beta({\cal D})$ are bound as
\begin{align}
&
%\myE_{\cal T^{\rm new} \sim \P{(\cal T)}}
%\myE_{\cal D \sim {\mathbb P}_{\phi^{\rm new}} }\myE_{\{\x,y\}\sim \cal T^{\rm new}}
{\mathbb E}\squarebrack{\round{\x^\top \hat{\beta}({\cal D})-y}^2}
\;\le\;  \delta+\round{1+\eps^2}\sum_{i=1}^kp_is_i^2\; ,
\label{eq:pred}
\end{align}
%and the same bound for the Bayes optimal estimator holds
%\begin{align*}
%&\mathbb{E}_{\cal T^{\rm new} \sim \P{(\cal T)}}\mathbb{E}_{\cal D \sim \cal T^{\rm new}}\mathbb{E}_{\{\x,y\}\sim \cal T^{\rm new}}\squarebrack{\round{\x^\top \hat{\beta}_{\rm Bayes}({\cal D})-y}^2}\\
%\le&\;  \delta+(1+\eps^2)\sum_{i=1}^kp_is_i^2\; .
%\end{align*}
if $\tau\ge \Theta\round{\log (k/\delta)/\Delta^4}$, 
where
the true meta-parameter is 
$\theta=\{(\w_i,s_i,p_i)\}_{i=1}^k$, 
the expectation is over the new task with model parameter $\phi^{\rm new}=(\beta^{\rm new},\sigma^{\rm new}) \sim {\mathbb P}_{\theta} $, training dataset ${\cal D}\sim{\mathbb P}_{\phi^{\rm new}} $, 
and test data $(\x,y)\sim {\mathbb P}_{\phi^{\rm new}}$. 
\end{thm}




%\begin{remark}
%%Denote the true regression vector for $\cal T^{\rm new}$ as $\beta^{\rm new}$. The MAP estimator estimate $\w_h$ with 
%The expected squared $\ell_2$ error is bounded as
%\begin{eqnarray*}
%%\mathop{\mathbb{E}}_{\cal T^{\rm new} \sim \P{(\cal T)}}\mathop{\mathbb{E}}_{\cal D \sim \cal T^{\rm new}}
%{\mathbb E} 
%\squarebrack{\esqnorm{\hat{\beta}({\cal D})-\beta^{\rm new}}} \; \le \;  \delta+\eps^2\sum\limits_{i=1}^kp_is_i^2,
%\end{eqnarray*}
%for both  Bayes optimal  and MAP estimators $\hat\beta({\cal D})$, 
%if $\tau\ge \Theta\round{\log (k/\delta)/\Delta^4}$. 
%%\begin{eqnarray*}
%%\mathop{\mathbb{E}}_{\cal T^{\rm new} \sim \P{(\cal T)}}\mathop{\mathbb{E}}_{\cal D \sim \cal T^{\rm new}}\squarebrack{\esqnorm{\hat{\beta}_{\rm Bayes}({\cal D})-\beta^{\rm new}}} \le \delta+\eps^2\sum\limits_{i=1}^kp_is_i^2.
%%\end{eqnarray*}
%\end{remark}

Note that the $\sum_{i=1}^k p_is_i^2$ term in \eqref{eq:pred} is due to the noise in $y$, and can not be avoided by any estimator. 
With an accurate meta-learning, we can achieve a prediction error arbitrarily close to this statistical limit, with $\tau=\BigO{\log k}$. 
Although both predictors achieve the same guarantee, Bayes optimal estimator achieves smaller training and test errors in Figure~\ref{fig:pred}, especially in challenging regimes with small data.
%parameter estimation error as expected. Further, the prediction error is also smaller. 

\begin{figure}[ht]
    \vskip -0.1in
    \begin{center}
    \subfigure[Training error]{\label{fig:train_err_32}\includegraphics[width=0.48\linewidth]{images/MAP_vs_Bayes_train_32.png}}
    \subfigure[Prediction error]{\label{fig:pred_err_32}\includegraphics[width=0.48\linewidth]{images/MAP_vs_Bayes_test_32.png}}
    \caption{Bayes optimal estimator achieves smaller errors for an example. Here, $k=32$, $d=256$, $\W^\top\W = \I_k$, $\s=\one_k$, $\p = \one_k/k$, and $\Pcal_\x$ and $\Pcal_\eps$ are standard Gaussian distributions. The parameters were learnt using the Meta-learning part of Algorithm~\ref{alg:estimate} as a continuation of simulations discussed in Appendix~\ref{sec:simulations}, where we provide extensive  experiments confirming our analyses.}
    \label{fig:pred}
    \end{center}
 %   \vskip -0.2in
\end{figure}

We show that $\tau= \Omega(\log k)$ training samples are necessary (even if the ground truths meta-parameter $\theta$ is known) to achieve error approaching this statistical limit. Let $ \Theta_{k,\Delta,\sigma}$ denote the set of all meta-parameters with $k$ components, satisfying $\|\w_i-\w_j\|_2 \geq \Delta$ for $i\neq j\in[k]$ and $s_i\leq \sigma$ for all $i\in [k]$. 
The following minimax lower bound shows that 
there exists a threshold scaling as $\BigO{\log k}$ below which no algorithm can achieve the fundamental limit of  $\sigma^2$, which is $\sum_{i=1}^k p_is_i^2$ in this minimax setting.  

\begin{remark}[Lower bound for prediction]\label{thm:lb-predict}
For any $\sigma,\Delta>0$, 
if $\tau =  \round{(1+\Delta^2)/\sigma^2}^{-1}\log(k-1)$, then 
    \begin{eqnarray}
    \inf_{\hat{y}}
    \sup_{\theta\in\Theta_{k,\Delta,\sigma}}
    \E{ \round{\hat{y}({\cal D},\theta)- y}^2} \; = \; \sigma^2 + \Omega\round{\Delta^2} \;,
    \end{eqnarray}
     where the minimization is over all measurable functions of the meta-parameter $\theta$ and the training data ${\cal D}$ of size $\tau$.
    \label{thm:lb}
\end{remark}



==> Meta-Learning Linear Regression_ k-Mixture/related.tex <==
\section{Related Work}
\label{sec:related} 








\begin{table*}[t]
\caption{Sample complexity for previous work in MLR to achieve small constant error on parameters recovery of the mixed linear regression problem. We ignore the constants and $\mathrm{poly}\log$ factors. Let $n,d$, and $k$ denote the number of samples, the dimension of the data points, and the number of clusters, respectively. 
\cite{yi2016solving} and~\cite{CL13} requires 
$\sigma_k$, the $k$-th singular value of some moment matrix. %and  %which is required by \cite{yi2016solving}. Let 
\cite{sedghi2016provable} requires $s_{\rm min}$, the $k$-th singular value of the matrix of the regression vectors.
 % in Sample Complexity ($\#$ Sample) and Running Time (Time). 
 Note that $1/s_{\rm min}$ and $1/\sigma_k$ can be infinite even when $\Delta>0$. \cite{zhong2016mixed} algorithm requires
 $\Delta_{\rm max}/\Delta_{\rm min} = \BigO{1}$ and
some spectral properties. } %Thus, our result is the first truly $\poly(k)$ time algorithm.
\label{tab:related}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}

\begin{tabular}{l c l} 
\toprule
{\bf References}  & {\bf Noise} & {\bf \# Samples $n$} \\
\midrule
\cite{CL13}  & Yes & $d^6 \cdot \poly(k, 1/\sigma_k)$  \\
\cite{yi2016solving}  & No & $d \cdot \poly(k,1/\Delta, 1/\sigma_k)$  \\
\cite{zhong2016mixed} & No  
%$\sigma_k(\M_2), \|\M_2\|,\|M_3\|_{\rm op}^{2/3}, \sum_{i\in[k]} \pi_i \|\w_i\|^2, (\sum_i \pi_i \|\w_i\|^{3})^{2/3}$ all have the same order in $d$
&$d \cdot \exp(k \log(k\log d)) $  \\
\cite{sedghi2016provable}  & Yes  & $d^3 \cdot \poly ( k, 1/s_{\rm min})$  \\
\cite{li2018learning}   & No & $d \cdot \poly(k/\Delta) + \exp(k^2 \log (k/\Delta) )$ \\
\cite{chen2019learning} & No  & $d \cdot \exp(\sqrt{k})\poly (1/\Delta)$  \\
%\cite{chen2019learning} & Yes & No & $d \cdot \exp(\sqrt{k}/\Delta^2)$ & $nd$ \\ \hline
%Ours & Yes & No & $d \cdot \poly(k)$ & $nd$ ? \\ \hline
\bottomrule
\end{tabular}

\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}




Meta-learning linear models 
have been studied in two contexts: mixed linear regression and multi-task learning.  

%Several algorithms with theoretical guarantees exist for multi-task learning, which addresses a more general setting. 

{\bf Mixed Linear Regression (MLR).}
When each task has only one sample, (i.e.~$t_i=1$), the problem has been widely studied.  
Prior work in MLR are summarized in Table~\ref{tab:related}. We emphasize that the sample  and time complexity of all the previous work either has a super polynomial dependency on $k$ (specifically at least $\exp(\sqrt{k})$) as in~\cite{zhong2016mixed, li2018learning, chen2019learning}), or depends on the inverse of the $k$-th singular value of some moment matrix as in~\cite{CL13, yi2016solving, sedghi2016provable}, which can be infinite.~\cite{chen2019learning} cannot achieve vanishing error when there is noise.

{\bf Multi-task learning.}  \cite{baxter2000model,ando2005framework,rish2008closed,orlitsky2005supervised} address a similar problem of finding 
%each parameter $\beta_i$ is assumed to lie on 
an unknown $k$-dimensional subspace, where all tasks can be accurately solved. 
The main difference is that 
all tasks have  the same  number   of examples, and the performance is evaluated on the  observed tasks used in training.  
Typical approaches use 
trace-norm to encourage low-rank solutions of the matrix $\begin{bmatrix}\hat\beta_i,\ldots,\hat\beta_n\end{bmatrix}\in{\mathbb R}^{d\times n}$. 
This is posed as a convex program~\cite{argyriou2008convex,harchaoui2012large,amit2007uncovering,pontil2013excess}.


Closer to our work is the streaming setting where $n$ tasks are arriving in an online fashion and one can choose how many examples to collect for each. \cite{balcan2015efficient} provides an online algorithm using a memory of size only $\BigO{k n + k d}$, but requires  
some tasks to have $t_i = \Omega\round{ dk/\epsilon^2}$ examples. 
In comparison, we only need  $t_H=\tilde\Omega(\sqrt{k})$ but use $\BigO{d^2+kn}$ memory.
\cite{bullins2019generalize} also use only small memory, 
but requires $\tilde\Omega\round{d^2}$ total  samples to perform the {\em  subspace estimation} under the setting studied in this paper.


%This allows  efficient methods of learning linear models to be seamlessly extended to non-linear models, and has been widely studied under the name of 

 
 
%Under the additive noise setting, existing  approaches require estimations and  operations of third order tensors, which require high sample and computational complexities.  \cite{CL13} constructs the tensor via tensor nuclear norm minimization, which requires $\BigO{\frac{d^6k^2}{\sigma_k^5\eps^2}}$ samples and $\BigO{n d^{12}}$ computations. \Zhao{Why not include the above result in the table. Sewoong: We were just separating out the cases where there is noise and the cases where there is no noise. We can decide how to present these results, when we know our final theorem.}
%\cite{sedghi2016provable} constructs the tensor using a score function, which only requires $\BigO{d^3k^4/(s^2\eps^2)}$ samples and $\BigO{nd^2}$ computations, where $s$ is the minimum singular value of the regression parameters $[\w_1, \cdots ,\w_k]$. % in the paper they say nd^2, but it is actually nkdL, with L number of initializations, which in not specified. 
%For a special case of $k=2$ components, \cite{CYC14} 



\noindent{\bf Empirical Bayes/Population of parameters.}
 A simple canonical setting of probabilistic meta-learning is when $\mathbb{P}_{\phi_i}$ is a univariate distribution (e.g. Gaussian, Bernoulli) and $\phi_i$ is the parameter of the distribution (e.g. Gaussian mean, success probability). 
 %which is drawn from a unknown prior $\mathbb{P}_\theta(\phi)$.
 Several related questions have been studied. In some cases, one might be interested in just learning the prior distribution $\mathbb{P}_\theta(\phi)$ or the set of $\phi_i$'s. For example, if we assume each student's score of one particular exam $x_i$ is a binomial random variable with mean $\phi_i$ (true score), given the scores of the students in a class, an ETS statistician~\cite{lord1969estimating} might want to learn the distribution of their true score $\phi_i$'s. Surprisingly, the minimax rate on estimating the prior distribution $\mathbb{P}_\theta(\phi)$ was not known until very recently~\cite{tian2017learning, vinayak2019maximum} even in the most basic setting where $\mathbb{P}_{\phi_i}(x)$ is  Binomial.

In some cases, similar to the goal of meta-learning, one might want to accurately estimate the parameter of the new task $\phi^{\rm new}$ given the new data $x^{\rm new}$, perhaps by leveraging an estimation of the prior $\mathbb{P}_\theta(\phi)$. This has been studied for decades under the \textit{empirical bayes} framework in statistics (see, e.g. the book by Efron~\cite{efron2012large} for an introduction of the field).


%In multi-task learning, the goal is slightly different. The goal is to learn a shared representation of the data that is universal, such that individual tasks can be learned over that representation . 


%We generalize and improve upon several theoretical results.

%{\bf Clustering Approach.}
%It is shown in~\cite{vempala2004spectral} that the centers of a Gaussian mixture model $\sum_{i=1}^k w_i\mathcal{N}(\mu_i, \I_d)$ can be learnt with separation $\Omega\round{{(k\log (d/w_{\min} ))}^{1/4}+ (\log (d/w_{\min}) )^{1/2}}$ in time polynomial in $k^{\BigO{k}}$ and $d$. 
%\begin{remark}
%It is shown in~\cite{chen2019learning} that any method of moments approach needs to look at at least $k$-th order moments to learn $\beta_i$ even when the separation $\min_{i\ne j}\|\beta_i-\beta_j\|_2$ is constant, which means the algorithm requires at least $\exp(k)$ samples. Intuitively, we can make all $\beta_i$ to be multiples of $\vvec\in \R^d$ to fool the moment algorithm.
%\end{remark}

%\Weihao{
%In the setting where $t\le \sqrt{k}$, we random pick a set of $\sqrt{k}/t$ people and let $\hat{\beta}_i$ be their estimates. We can check the norm of the mean of $\hat{\beta}_i$ and their average distance to their mean. If the average distance to the mean is small, we know that they are from the same $w$ and thus should be grouped together. With probability $(1/k)^{\sqrt{k}/t}$, we obtain a set of people that belong to the same $w$, and the set of people has a total of $\sqrt{k}$ samples. Repeating this procedure a certain number of times, we are back to the $t=\sqrt{k}$ setting.}

%\noindent{\bf Crowdsourcing.}
% Crowdsourcing models are special case of our models, but no theory known, only heuristics. 








\section{Discussion}
\label{sec:discussion} 

We investigate how we can meta-learn when we have multiple tasks but each with a small number of labelled examples. This is also known as a few-shot supervised learning setting. When each task is a linear regression, we propose a novel spectral approach and show that we can leverage past experience on small data tasks to accurately learn the meta-parameters and predict new tasks. 

When each task is a logistic regression coming from a mixture model, then our algorithm can be applied seamlessly. 
However, the notion of  separation $\Delta = \min_{i\neq j} \|\w_i-\w_j\|_2$ does not capture the dependence on the statistical complexity. Identifying the appropriate notion of complexity 
 on the groundtruths meta-parameters is an interesting research question. 

The subspace estimation algorithm requires a total number of $\tilde\Omega(dk^2)$ examples. It is worth understanding whether this is also necessary. 
% information theoretically.

Handling the setting where $\Pcal_\x$ has different covariances in different tasks is a challenging problem. There does not seem to exist an unbiased estimator for $\W$. Nevertheless,~\cite{li2018learning} study the $t=1$ case in this setting and come up with an exponential time algorithm. Studying this general setting and coming up with a polynomial time algorithm for meta-learning in a data constrained setting is an interesting direction.




Our clustering algorithm requires the existence of medium data tasks with $t_H = \Omega(\sqrt{k})$ examples per task. It is worth investigating whether there exists a polynomial time and sample complexity algorithms that learns with $t_H = o(\sqrt{k})$. We conjecture that with the techniques developed in the robust clustering literature~\cite{diakonikolas2018list, hopkins2018mixture, kothari2018robust}, it is possible to learn with $t_H = o(\sqrt{k})$ in the expense of larger $n_H$, and higher computation complexity. For a lower bound perspective, it is worth understanding the information theoretic trade-off between $t_H$ and $n_H$ when $t_H=o(\sqrt{k})$.

\section{Acknowledgement}
Sham Kakade acknowledges funding from the Washington Research Foundation for Innovation in Data-intensive Discovery, and the NSF Awards CCF-1637360, CCF-1703574, and CCF-1740551.
